Parallelizing the Symbolic Manipulation Program FORM Part I: Workstation Clusters and Message Passing

The present paper is the first of a series of papers reporting on the parallelization of the symbolic manipulation program FORM on different parallel architectures. Part I deals with workstation clusters using dedicated network hardware and the messages passing libraries (MPI and PVM). After a short introduction to the sequential version of FORM a detailed analysis of the different platforms used is given and the structure of the parallel version of FORM is explained. The forthcoming part II will describe the parallelization of FORM on SMP (symmetrical multi-processing) architectures.

==> src/profile.tex <==
\begin{verbatim}
%time     seconds  cum %   cum sec  procedure

 20.2    501.6201   20.2    501.62 Normalize             G
 13.4    331.3018   33.6    832.92 Compare               S
  8.5    210.6748   42.1   1043.60 PutOut                S
  5.7    141.9512   47.8   1185.55 StoreTerm             S
  3.4     83.7432   51.2   1269.29 TestSub               G
  3.0     73.2539   54.1   1342.54 MergePatches          S
  2.9     72.4668   57.0   1415.01 InsertTerm            G

  0.9     21.7793   87.5   2171.72 EndSort               S

\end{verbatim}

